Few-Shot Learning with Intra-Class Knowledge Transfer

We consider the few-shot classification task with an unbalanced dataset, in which some classes have sufficient training samples while other classes only have limited training samples. Recent works have proposed to solve this task by augmenting the training data of the few-shot classes using generative models with the few-shot training samples as the seeds. However, due to the limited number of the few-shot seeds, the generated samples usually have small diversity, making it difficult to train a discriminative classifier for the few-shot classes. To enrich the diversity of the generated samples, we propose to leverage the intra-class knowledge from the neighbor many-shot classes with the intuition that neighbor classes share similar statistical information. Such intra-class information is obtained with a two-step mechanism. First, a regressor trained only on the many-shot classes is used to evaluate the few-shot class means from only a few samples. Second, superclasses are clustered, and the statistical mean and feature variance of each superclass are used as transferable knowledge inherited by the children few-shot classes. Such knowledge is then used by a generator to augment the sparse training data to help the downstream classification tasks. Extensive experiments show that our method achieves state-of-the-art across different datasets and $n$-shot settings.

==> rebuttal_content.tex <==
\section{Visualization}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{pics/class_tsne.png}
\caption{TSNE visualization of class samples, input seed samples for the generator, and generated samples. Generated samples are distributed close to the class mean providing better prototypes to the classifier.}
\label{fig:class_tsne}
\end{figure}

Figure \ref{fig:class_tsne} shows that the augmented samples belong perfectly to the same classes as the input seeds while being away from the decision boundaries.  The result indicates that the statistical information inherited from super classes can help ensure that the generated samples belong to the same class as the seed. This is because the classes belonging to the same super class share similar statistics and thereby transferable information.  Such statistical information can be treated as the class prototype.  The prototype tells the generator what the object should roughly look like, and the few-shot samples will give the generator detailed information to fine-tune the generated samples.  The result also shows that the regressor trained on many-shot classes can predict meaningful class means for few-shot classes.  There is no issue with unbalanced data between the estimated many-shot and few-shot class means.
